Sparsity and Privacy in Secret Sharing: A Fundamental Trade-Off

This work investigates the design of sparse secret sharing schemes that encode a sparse private matrix into sparse shares. This investigation is motivated by distributed computing, where the multiplication of sparse and private matrices is moved from a computationally weak main node to untrusted worker machines. Classical secret-sharing schemes produce dense shares. However, sparsity can help speed up the computation. We show that, for matrices with i.i.d. entries, sparsity in the shares comes at a fundamental cost of weaker privacy. We derive a fundamental tradeoff between sparsity and privacy and construct optimal sparse secret sharing schemes that produce shares that leak the minimum amount of information for a desired sparsity of the shares. We apply our schemes to distributed sparse and private matrix multiplication schemes with no colluding workers while tolerating stragglers. For the setting of two non-communicating clusters of workers, we design a sparse one-time pad so that no private information is leaked to a cluster of untrusted and colluding workers, and the shares with bounded but non-zero leakage are assigned to a cluster of partially trusted workers. We conclude by discussing the necessity of using permutations for matrices with correlated entries.

==> sparse_perfect_IT_privacy.tex <==
In this section, we propose a one-sided private and sparse matrix multiplication scheme, where the matrix $\bfB$ is publicly made available from the {\master}. Moreover, we tackle the problem of hiring {\workers} from fully unknown and untrusted providers. 


\begin{figure*}[!t]
    \centering
    \resizebox{.95\textwidth}{!}{\input{./figures/frac_rep_perfect_privacy}}
    \caption{The two non-communicating clusters, namely the untrusted and partly trusted one are illustrated on the left and right hand side, respectively. The {\workers} of the untrusted cluster $w_1^{\text{u}}, w_2^{\text{u}}, \dots, w_{\noworkersuntrusted}^{\text{u}}$ get each $\stragglerun$ tasks (created as in~\cref{subsec:task_distrib}) that leak nothing about the input matrix. On the other hand, each {\worker} of the partly trusted cluster $w_1^{\text{t}}, w_2^{\text{t}}, \dots, w_{\noworkerstrusted}^{\text{t}}$ gets $\stragglertr$ tasks that leak some information about the input matrix. Every {\worker} has to multiply the designated matrices with the public matrix $\bfB$ and then sent each computation back to the {\master}.}
    \label{fig:fractional_repetition_sparse}
\end{figure*}

\subsection{The clustering model}\label{subsec:clustering}
The {\master} hires external $\nbworkers$ workers, where $\nbworkers = \noworkersuntrusted + \noworkerstrusted$, that are grouped into two clusters: 
\begin{enumerate}
    \item \emph{Untrusted cluster:} The cluster consists of $\noworkersuntrusted$ workers, $w_1^u$, for $i = 1, \dots, \noworkersuntrusted$. The workers of this cluster are fully untrusted and they can all collude and therefore no leakage of information about $\bfA$ should be tolerated, i.e., perfect privacy. 
    \item \emph{Partly trusted cluster:} This cluster is composed of $\noworkerstrusted$ partly trusted {\workers} $w_i^t$, for $i=1,\dots, \noworkerstrusted$, that are partly known to the {\master} and up to $z$ {\workers} can collude. A small amount of information about $\bfA$ can be leaked if necessary.
\end{enumerate}
The grouping of {\workers} into two \emph{non-communicating} has practical relevance since the untrusted cluster can represent an externally hired computational node pool offered by a single provider, while the partly trusted cluster might represent a locally available computing pool, that can be partly trusted, but not fully. We will combine the sparse dependent one-time pad as specified in~\cref{lemma:sparse_perfect_ot_pad} with the cyclically shifted task assignment~\cite{coded_sparse_matrix_leverages_partial_stragglers},\cite{el2010fractional} to obtain a straggler-resilient coded computing scheme. 

\subsection{Task distribution and straggler mitigation}
\label{subsec:task_distrib}

\cref{fig:fractional_repetition_sparse} depicts the task distribution strategy for the scenario provided in~\cref{subsec:clustering}. The {\master} observes the input matrix $\bfA \in \F_q^{\nrowsA \times \ncolsA}$ and creates a matrix $\bfR \in \F_q^{\nrowsA \times \ncolsA}$ of the same size as described in~\cref{eq:dependent_on_0,eq:dependent_on_nz} for the special case $\pz = \pnz =p$ and $\pext = \frac{1-p}{q-1}$. The {\master} splits the padded matrix $\bfA + \bfR$ row-wise into $\noworkersuntrusted$ sub-matrices and splits the padding matrix $\bfR$ into $\noworkerstrusted$ sub-matrices as follows 
\begin{align*}
\bfA+\bfR &= \begin{pmatrix}
(\bfA+\bfR)_1\\ 
(\bfA+\bfR)_2\\ 
\vdots\\
(\bfA+\bfR)_{\noworkersuntrusted}
\end{pmatrix} 
&\bfR = \begin{pmatrix}
\bfR_1\\ 
\bfR_2\\
\vdots\\
\bfR_{\noworkerstrusted}
\end{pmatrix}\,,
\end{align*}
where $(\bfA+\bfR)_i \in \F_q^{\frac{\nrowsA}{\noworkersuntrusted}\times \ncolsA}$ for $i \in [\noworkersuntrusted]$ and $\bfR_j \in \F_q^{\frac{\nrowsB}{\noworkerstrusted}\times \ncolsB}$ for $j \in [\noworkerstrusted]$. Then, the {\master} sends to every {\worker} $w_i^{\text{u}}$ of the untrusted cluster a sub-matrix $\bfT_{i, 1}^{\text{u}} = (\bfA + \bfR)_i$ for $i\in [\noworkersuntrusted]$ and to to every {\worker} $w_k^{\text{t}}$ of the partly trusted cluster the {\master} assigns the sub-matrices $\bfT_{k, 1}^{\text{t}} = \bfR_k$ for $k \in [\noworkerstrusted]$. As illustrated in~\cref{fig:fractional_repetition_sparse}, the collection of these sub-matrices is referred to as the first \emph{layer} of computation tasks.


The {\master} then assigns the computation tasks of the other layers following a cyclic shifting strategy as
\begin{align*}
\bfT^{\text{u}}_{(i \mod \noworkersuntrusted)+1,j} &= \bfT^{\text{u}}_{i,j-1},\quad i \in [\noworkersuntrusted], j \in [\stragglerun] \setminus \{1\},\\
\bfT^{\text{t}}_{(k \mod \noworkerstrusted)+1, b} &= \bfT^{\text{t}}_{k, b-1},\quad k \in [\noworkerstrusted], b \in [\stragglertr] \setminus \{1\}.
\end{align*}
The matrix $\bfB$ is published (by the {\master} or it might be public information) and all the {\workers} can access it. Then every {\worker} of the untrusted cluster $w_i^{\text{u}}$ for $i\in[\noworkersuntrusted]$, needs to multiply the sub-matrices of all the layers $\{\bfT^{\text{u}}_{i,j}\}_{j=1}^{\stragglerun}$ with the public matrix $\bfB$, i.e., $\cW^{\text{u}}_i = \{(\bfT^{\text{u}}_{i,j},\bfB)\}_{j=1}^{\stragglerun} $. Similarly, the workers of the partly trusted cluster $w_k^{\text{t}}$ for $k\in[\noworkerstrusted]$ have the following multiplication tasks in $\cW_k^{\text{t}} = \{(\bfT^{\text{t}}_{k,b},\bfB)\}_{b=1}^{\stragglertr}$. After the {\workers} are done with each task, they send the results back to the {\master}. %
Our task assignment strategy allows for resiliency against both partial and full stragglers, which will be quantified in~\cref{thm:main}. 

\begin{theorem}\label{thm:main}
If the cyclic shift assignment strategy explained above is used and (all) the {\workers} of the untrusted cluster collude they will still learn nothing about the private matrix $\bfA$, i.e., $\mutinf(\{\rvT_{i,j}^{\text{u}}\}_{i\in[\noworkersuntrusted],j\in[\stragglerun]};\rvA) = 0.$
If up to $z$ {\workers} of the partly trusted cluster collude, then the leakage about the input matrix $\bfA$ is quantified by 
\begin{equation}\label{eq:colluding_trusted}
    \mutinf(\{\rvT^{\text{t}}_{i,j}\}_{i\in\cZ, j\in [\stragglertr]};\rvA) = \min\left\{\dfrac{\stragglertr z}{\noworkerstrusted}, 1\right\}\cdot m \cdot n \cdot \leakage{1}.
\end{equation}
The {\master} is able to reconstruct the desired computation after receiving any $K^{\text{u}} \triangleq \frac{-\stragglerun^2 +\stragglerun(2\noworkersuntrusted-1)}{2} +1$ and any $K^{\text{t}} \triangleq \frac{-\stragglertr^2 +\stragglertr(2\noworkerstrusted-1)}{2} +1$ responses from the {\workers} of the untrusted and partly trusted clusters, respectively. %
In addition, if full stragglers are contacted, up to $\stragglerun - 1$ and $\stragglertr - 1$ stragglers can be tolerated from the respective clusters.
\end{theorem}
\begin{proof}
    The proof is provided in~\cref{proof4}.
\end{proof}

In~\cref{thm:main} the privacy aspect of the scheme was quantified and in~\cref{lemma:sparse_perfect_ot_pad}, the trade-off between privacy and sparsity for the scheme was introduced. Therefore, for a given maximum affordable privacy leakage $\varepsilon$, the only constraint imposed to the {\master} is $\mutinf(\{\rvT^{\text{t}}_{i,j}\}_{i\in\cZ, j\in [\stragglertr]};\rvA) \leq \varepsilon$. 
Hence, we have 
\begin{equation}\label{eq:individual_leakage}
    \leakage{2} \leq \dfrac{\bar{\varepsilon}\entropy(\Aij)}{\min\{\frac{\stragglertr z}{\noworkerstrusted},1\}}.
\end{equation} 
Then maximum sparsity levels allowed for the sub-matrices are given by
\begin{align*}
    \sar &= p^\star, \quad \text{ and } \quad\sr = p^* \frac{sq-1}{q-1}+\frac{1-s}{q-1},
\end{align*}
where 
\begin{equation}
    \label{eq:pstar}
    p^* = \max_{\mutinf(\{\rvT^{\text{t}}_{i,j}\}_{i\in\cZ, j\in [\stragglertr]};\rvA)\leq \varepsilon} p.
\end{equation}
We plot in~\cref{fig:my_label} the maximum value of $p^*$ versus the number of colluding {\workers} of partly trusted cluster $z$. The plots are provided for a varying choice of maximum relative leakage tolerated. Observe that $p^*$ decreases with $z$ as more {\workers} collude and can have access to a bigger portion of resemblance to the private matrix $\bfA$. As expected, decreasing the relative leakage $\bar{\varepsilon}$, forces the maximum value for $p^*$ to drop, meaning that the sparsity levels $\sr, \sar$ should have lower values. Using the terminology in~\cref{def:spmm}, we constructed a sparse and private matrix multiplication with $(\shares = \noworkersuntrusted\stragglerun+\noworkerstrusted\stragglertr, \sigma=\min\{\stragglerun-1,\stragglertr-1\}, \varepsilon_1 = \leakage{2}, \bar{\varepsilon}_2 = 1, s_1\approx p^*, s_2 = \sbm)$.\marvin{We can move this in the beginning of this section or not refer at all, since it is not cooked for the clustering case I believe.}

